Privacy Threats Against Federated Matrix Factorization

Matrix Factorization has been very successful in practical recommendation applications and e-commerce. Due to data shortage and stringent regulations, it can be hard to collect sufficient data to build performant recommender systems for a single company. Federated learning provides the possibility to bridge the data silos and build machine learning models without compromising privacy and security. Participants sharing common users or items collaboratively build a model over data from all the participants. There have been some works exploring the application of federated learning to recommender systems and the privacy issues in collaborative filtering systems. However, the privacy threats in federated matrix factorization are not studied. In this paper, we categorize federated matrix factorization into three types based on the partition of feature space and analyze privacy threats against each type of federated matrix factorization model. We also discuss privacy-preserving approaches. As far as we are aware, this is the first study of privacy threats of the matrix factorization method in the federated learning framework.

==> old_text.tex <==
\begin{abstract}
Federated Learning (FL) is an emerging technology, which bridges the data silos and builds machine learning models without compromising privacy and security. It can improve model performance by utilizing the auxiliary features from other parties. 
The cross-feature technique that explicitly learns interactions among features is popularly utilized to improve models’ expressiveness in many machine learning tasks, such as recommender systems. Yet, due to the privacy concern and communication cost, existing algorithms are not able to handle cross-features under the FL setting. Therefore, in this paper, firstly, we propose the Federated Collective Matrix Factorization (FedCMF), which models high order feature interactions within each party and interactions between isolated parties. FedCMF builds the model by exchanging parameters between parties, without data leaving their own repositories. For preserving data privacy, it also adopts a secure computation protocol, which is based on the secret sharing and homomorphic encryption (HE) techniques. The protocol protects FedCMF against model inversion attack and data reconstruction attack during the parameter exchanging procedures. Secondly, we propose a secure sparse inner product protocol for FedCMF to deal with high-dimensional sparse features, which commonly exist in recommender systems. The communication and computation cost is dramatically reduced when training the FedCMF model with encrypted parameters. 
\end{abstract}

\section{Introduction}
Federated learning (FL) enables multiple parties to collaboratively train machine learning models without exposing ones' own data. It addresses the data silos and privacy problem together. 
%Based on how data is distributed among various parties in the feature and sample ID space, FL is classified into horizontally federated learning, vertically federated learning and federated transfer learning~\cite{yang2019federated}. 
In this paper, we consider a typical federated learning scenario in the recommender systems. 
%vertically federated learning (VFL), where datasets from the collaborated parties share the same sample ID space but differ in feature space.
Taking the collaboration between a movie recommender and a data provider as an example, the intersection of their user space is large. The recommender records the user’s rating, browsing and watching history of the recommended movies, while the data provider owns the demographic information. Their feature spaces are very different. We propose a method to integrate the features of these two parties in a secure and privacy-preserving way and improve the recommendation performance.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{kdd2020/figure_FedCMF.pdf}
%     \caption{Overview of the Federated Factorization Machine (FedCMF). In this example, two parties collaboratively learn recommender model with their data kept locally. The FedCMF explicitly captures the feature interaction within each party and between two parties in a privacy-preserving way, where only the model parameters and intermediate results are transmitted between parties instead of the raw data.}
%     \label{fig_intro_overview}
% \end{figure}


The feature interaction is a widely used method to integrate features and increase the models’ expressiveness. For example, the movie recommender has features about the movie genres, and the data provider has user gender information. For instance, through modeling the interaction between ``gender-male'',  ``gender-female'', ``genres-romance'' and ``genres-adventure'' features, we can capture the preferences of different user groups, such as ``female on  romance'' and ``male on adventure''. Learning interactions among features is significant in improving the models’ performance. In the federated learning setting, these features are stored in the movie recommender and data provider, respectively. They could not leave their own data repository and never be transmitted due to privacy concerns. Previous learning algorithms, which build a model on centrally collected data, are not able to model the interactions between features distributed on these two parties. Besides, although we can model the feature interaction through the weight parameters of feature pairs and learning the model by exchanging weight parameters as previous FL algorithms did, the communication cost could be extremely high. Taking the second-order feature interaction as an example, the cost is $O(d_A\times d_B)$, where $d_A$ and $d_B$ are the feature dimensions. It is unacceptable with iterative optimization algorithms, which is widely adopted in FL. Furthermore, to avoid information leakage, the weight parameters are usually encrypted by the encryption algorithm. The bit lengths of the parameters increase in the encrypted space. Therefore, the communication cost further increases. 

In this paper, we propose the \textbf{Federated Collective Matrix Factorization} (FedCMF) algorithm. As shown in Figure ~\ref{fig_intro_overview}, the FedCMF explicitly captures the feature interactions inside each party as well as between two parties in a privacy-preserving way. Only the model parameters and intermediate results are transmitted between parties instead of the raw data. As we prove in the following sections, the communication cost between two parties is at most $O(d\times d')$, where $d'$ is a hyper-parameter and much smaller than the original dimensions $d\in \{d_A, d_B\}$. The FedCMF is based on traditional collective matrix factorization (CMF), which is proposed in ~\cite{rendle2010factorization}. Traditional CCMF parameterizes the weight of the feature interaction as the inner product of the embedding vectors of the constituent features. By learning an embedding vector for each feature, traditional CCMF can estimate the weight for any interacted features. However, traditional CCMF is not designed for decentralized data. In other words, all the interacted features should be collected together on a central server, then the traditional CMF can start to learn the model. For the federated learning setting, we propose a federated collective matrix factorization by reformulating the objective function of the traditional CCMF. The FedCMF exchanges embedding vectors and their partial gradients between parties to capture the feature interactions, without collecting raw data from isolated parties. 

Nonetheless, exchanging the clear-text intermediate results in the FedCMF results in high privacy risks and is vulnerable to model inversion attack and data reconstruction attack. Theoretically, we prove that the model and raw data could be fully reconstructed by inserting a few known instances to the other party. To enhance the model security, we propose a secure computation protocol, where the intermediate results are encrypted by secret sharing and exchanged with MPC protocol~\cite{7958569}. With the secure protocol, no bit of information will be leaked between parties. For the tasks that have high-dimensional sparse features, to protect the positional information of the non-null features, the secure computation protocol has to be conducted over all features, including the zero-value (and blank) features. It is not practical. Therefore, we further propose a secure sparse inner product protocol based on homomorphic encryption (HE). The secure computation is only conducted on non-null features, and the intermediate results that updated by the non-null features are encrypted by homomorphic encryption. The communication cost further decreases to $O(\hat{d}\times d')$, where $\hat{d}\in \{\hat{d}_A, \hat{d}_B\}$ is the number of non-null features in the instance. In most high-dimensional sparse cases, the $\hat{d}$ is much smaller than the original dimension $d$ in each instance. 


In summary, our contributions are three folds:
\begin{itemize}
    \item We propose a new FedCMF algorithm that models feature interactions between parties with small communication cost and is secure against model inversion attack and data reconstruction attack.
    \item We also propose a secure sparse inner product protocol to handle high-dimensional sparse features, which commonly exists in recommender systems and has not been studied in federated learning so far.
	\item We evaluate the FedCMF over three real-world datasets, showing fast convergence and promising performance improvement.
\end{itemize}

In the following parts of this article, section~\ref{problemdefinition} gives a formal definition of federated learning with feature interactions. In section~\ref{vfCMF}, we introduce the traditional factorization machine and the federated factorization machine. In section~\ref{securevfCMF}, first of all, we theoretically prove the information leakage when FedCMF transmits clear-text intermediate results. Then, we introduce secure computation protocols. In section~\ref{exp}, we conduct experiments to evaluate the proposed FedCMF. We summary the related work in section~\ref{relatedwork} and conclude the paper in section~\ref{conclusion}.



% In this paper, we assume that two parties $P^{A}$ and $P^{B}$ collaboratively learn a machine learning model. $P^{A}$ has data source $\mathbf{R}\in \mathrm{R}^{N_u,N_v}$ and $P^{B}$ has data source $\mathbf{U} \in \mathrm{X}^{N_u, N_m}$ for $N_u$ common users, $N_v$ items of A and $N_m$ items of B. The collective matrix factorization method FedCMF is defined as follows:
% \begin{align*}
%     & \mathbf{R} \sim \mathbf{P^T Q}, \\
%     & \mathbf{X} \sim \mathbf{P^T U}
% \end{align*}

% $\mathbf{X}^{A} =\{\mathbf{x}^{A}_1,\mathbf{x}^{A}_2,\cdots, \mathbf{x}^{A}_{n_a}\}$ has $n_a$ instances, and each instance $\mathbf{x}^{A}_i\in\mathbb{R}^{d_A}$ is a $d_A$ dimension feature vector. $\bm{Y}_A = \{y_1, y_2, \cdots, y_{n_a}\}$, where $y_i\in\mathbb{R}$, are the labels of the instances. $P^{B}=\{\mathbf{X^{B}}\}$ has the other feature sets. $\mathbf{X}^{B} =\{\mathbf{x}^{B}_1,\mathbf{x}^{B}_2,\cdots, \mathbf{x}^{B}_{n_b}\}$ has $n_b$ instances, and each instance $\mathbf{x}^{B}_i\in\mathbb{R}^{d_B}$ is a $d_B$ dimension feature vector. The numbers of instances in each party could be unequal. The goal is to explicitly model the interactions between features of two parties and learn a predictive function:

% where $f_{\mathbf{w_A}}(\mathbf{x}^A)$ and $f_{\mathbf{w_B}}(\mathbf{x}^B)$ are partial functions that capture the interactions between features within party A and B respectively, $f_{\mathbf{w_{AB}}}([[\mathbf{x}^A]];[[\mathbf{x}^B]])$ captures the feature interactions between party A and B. In the federated learning setting, the data must be kept locally. Therefore, the weights of feature interactions should be learned in a privacy-preserving manner without data leakage, $[[\cdot]]$ here is the privacy-preserving method. The final objective function is
% \begin{equation*}
%     \mathop{\arg\min}_{\mathbf{w}} \sum_{i=1}^n l(r_ij - \mathbf{p}_i^T \mathbf{q}_j) + \Omega(\mathbf{w}),
% \end{equation*}
% where $l(\cdot)$ is the loss function, $\Omega(\cdot)$ is the regularization function, $n$ is number of instances whose indices are matched in both parties. 


% \section{Problem Definition}\label{problemdefinition}
% In this paper, we assume that two parties $P^{A}$ and $P^{B}$ collaboratively learn a machine learning model. $P^{A}$ has data source $\mathbf{R}\in \mathrm{R}^{N_u,N_v}$ and $P^{B}$ has data source $\mathbf{U} \in \mathrm{X}^{N_u, N_m}$ for $N_u$ common users, $N_v$ items of A and $N_m$ items of B. The collective matrix factorization method FedCMF is defined as follows:
% \begin{align*}
%     & \mathbf{R} \sim \mathbf{P^T Q}, \\
%     & \mathbf{X} \sim \mathbf{P^T U}
% \end{align*}

% $\mathbf{X}^{A} =\{\mathbf{x}^{A}_1,\mathbf{x}^{A}_2,\cdots, \mathbf{x}^{A}_{n_a}\}$ has $n_a$ instances, and each instance $\mathbf{x}^{A}_i\in\mathbb{R}^{d_A}$ is a $d_A$ dimension feature vector. $\bm{Y}_A = \{y_1, y_2, \cdots, y_{n_a}\}$, where $y_i\in\mathbb{R}$, are the labels of the instances. $P^{B}=\{\mathbf{X^{B}}\}$ has the other feature sets. $\mathbf{X}^{B} =\{\mathbf{x}^{B}_1,\mathbf{x}^{B}_2,\cdots, \mathbf{x}^{B}_{n_b}\}$ has $n_b$ instances, and each instance $\mathbf{x}^{B}_i\in\mathbb{R}^{d_B}$ is a $d_B$ dimension feature vector. The numbers of instances in each party could be unequal. The goal is to explicitly model the interactions between features of two parties and learn a predictive function:

% where $f_{\mathbf{w_A}}(\mathbf{x}^A)$ and $f_{\mathbf{w_B}}(\mathbf{x}^B)$ are partial functions that capture the interactions between features within party A and B respectively, $f_{\mathbf{w_{AB}}}([[\mathbf{x}^A]];[[\mathbf{x}^B]])$ captures the feature interactions between party A and B. In the federated learning setting, the data must be kept locally. Therefore, the weights of feature interactions should be learned in a privacy-preserving manner without data leakage, $[[\cdot]]$ here is the privacy-preserving method. The final objective function is
% \begin{equation*}
%     \mathop{\arg\min}_{\mathbf{w}} \sum_{i=1}^n l(r_ij - \mathbf{p}_i^T \mathbf{q}_j) + \Omega(\mathbf{w}),
% \end{equation*}
% where $l(\cdot)$ is the loss function, $\Omega(\cdot)$ is the regularization function, $n$ is number of instances whose indices are matched in both parties. 

% \section{Clear-text Federated Factorization Machine}\label{vfCMF}
% CMF is widely used and very effective at modeling feature interactions. In this section, We firstly give a brief introduction to the traditional CMF algorithm. It collects all the data together and learns the CMF model. Then, we explain the federated collective matrix factorization (FedCMF) algorithm that is able to learn the CMF model collaboratively without data leaving its own repository.

% \subsection{Traditional Collective Matrix Factorization}
% In traditional CMF, we have $\mathbf{x}=(\mathbf{x}^A, \mathbf{x}^B)$. Taking the second-order interaction as example, the CMF prediction function is defined as:
  
% \begin{equation*}%\label{CMF_prediction}
%     f(\mathbf{x}) = \langle \mathbf{w}, \mathbf{x} \rangle + \sum_{i<j} \langle \mathbf{v_i}, \mathbf{v_j} \rangle x_ix_j,
% \end{equation*}
% where the model parameters that have to be estimated are $\mathbf{w} \in \mathbb{R}^{d+1}$, $\mathbf{v}_i\in \mathbb{R}^{d’}$ is the embedding vector for the $i$th feature, $\langle \cdot ,\cdot \rangle $ is the dot product of two vectors of size $d'$.

% The dot product of $\langle \mathbf{v_i}, \mathbf{v_j} \rangle$ models the feature interaction between $x_i$ and $x_j$. Consider an $l_2$-norm regularization function
% $\Omega(\mathbf{w}, \mathbf{V}) = ||\mathbf{w}||_2^2 +||\mathbf{V}||_2^2,
% $ where $\mathbf{V} \in \mathbb{R}^{d \times d'}$. CMF loss function is defined as
% \begin{equation*}\label{CMF_loss}
%     l(\mathbf{w}, \mathbf{V}):= \frac{1}{2n} \sum_{l=1}^n (y_l - f(\mathbf{x}_l))^2 + \frac{\alpha}{2}\Omega(\mathbf{w}, \mathbf{V}),
% \end{equation*}
% where $\alpha > 0$ is a hyper-parameter. 

% \subsection{Federated Collective Matrix Factorization}

% In the federated learning setting, two parties keep their raw data locally. Two parties need to match the shared common instances by exchanging the sample IDs. After finding the inner join of the two data sets, the two parties can start federated model training. The CMF prediction function over two parties is
% \begin{equation}\label{fedCMF_prediction}
%     f([\mathbf{x}^{A}; \mathbf{x}^{B}]) = f(\mathbf{x}^{A}) + f(\mathbf{x}^{B}) + \sum_{i,j} \langle \mathbf{v}_i^{A}, \mathbf{v}_j^{B} \rangle x_{i}^{A} x_{j}^{B},
% \end{equation}
% where 
% \begin{equation}\label{eq_fxa}
%     f(\mathbf{x}^{A}) = \langle \mathbf{w}^{A}, \mathbf{x}^{A} \rangle + \sum_{i<j} \langle \mathbf{v}_i^{A}, \mathbf{v}_j^{A}\rangle x_i^{A} x_j^{A},
% \end{equation}
% and
% \begin{equation}\label{eq_fxb}
%     f(\mathbf{x}^{B}) = \langle \mathbf{w}^{B}, \mathbf{x}^{B} \rangle + \sum_{i<j} \langle \mathbf{v}_i^{B}, \mathbf{v}_j^{B}\rangle x_i^{B} x_j^{B}.
% \end{equation}
% In Equation~\ref{fedCMF_prediction}, $f(\mathbf{x}^{A})$ and $f(\mathbf{x}^{B})$ capture the feature interactions within party A and B respectively, $\sum_{i,j} \langle \mathbf{v}_i^{A}, \mathbf{v}_j^{B} \rangle x_{i}^{A} x_{j}^{B}$ captures the feature interactions between party A and B. We define the CMF loss function over two parties as
% \begin{equation*}
%     \begin{aligned}\label{fedCMF_loss}
%     & l(\mathbf{w}, \mathbf{V})
%     & := \frac{1}{2n} \sum_{i=1}^{n} (y_i - f([\mathbf{x}_i^{A}; \mathbf{x}_i^{B}]))^2 + \Omega(\mathbf{w}, \mathbf{V}), 
% \end{aligned}
% \end{equation*}
% where $n$ is the batch size. 

